Resource-constrained Project Scheduling with Time-of-Use Energy Tariffs and Machine States: A Logic-based Benders Decomposition Approach

In this paper, we investigate the Resource-Constrained Project Scheduling Problem (RCPSP) with Time-of-Use (TOU) energy tariffs and machine states, a variant of RCPSP for production scheduling, where energy price is part of the criteria and one highly energy-demanding machine can be in one of the following three states: proc, idle, or off. The problem involves scheduling all tasks, respecting precedence constraints and resource limitations, while minimizing the combination of the overall makespan and the Total Energy Cost (TEC), which varies according to the TOU tariffs, which can take negative values. We propose two novel approaches to solve it: a monolithic Constraint Programming (CP) approach and a Logic-Based Benders Decomposition (LBBD) approach. The latter combines a master problem handling the energy cost solved using Integer Linear Programming (ILP) with a subproblem handling the RCPSP, resolved using CP. Both approaches outperform the monolithic compact ILP counterpart, but the LBBD significantly outperforms the monolithic CP in most cases, especially when the makespan criterion is not included in the objective function, solving to optimality instances with up to 480 tasks. Finally, we propose a way to generalize our LBBD approach to other problems sharing similar characteristics, and applied it to various problems, such as an RCPSP with blocking times & total weighted tardiness criterion, or a flexible job shop.

==> fig/interval_state_graph.tex <==
{
\newcommand{\ImNumInts}{17} % number of intervals
\newcommand{\ImNumModes}{3} % number of rows

\newcommand{\ImGridVert}{0.65} % size of the grid cell
\newcommand{\ImGridHor}{4.5} % size of the grid cell
\newcommand{\ImNodeWidth}{4pt}

\newcommand{\ImOffIdx}{1}
\newcommand{\ImProcIdx}{2}
\newcommand{\ImIdleIdx}{3}

\definecolor{ImClrNode}{RGB}{95,171,182}

\newcommand{\myNode}[1]{v_{#1}}

\definecolor{ImClrLightgray}{RGB}{220,220,220}
\definecolor{ImClr1}{RGB}{199,229,242}
\definecolor{ImClr2}{RGB}{95,171,182}
\definecolor{ImClr3}{RGB}{187,217,118}
\definecolor{ImClr4}{RGB}{244,209,73}
\definecolor{ImClr5}{RGB}{235,121,107}

\definecolor{ImClrGreen}{RGB}{0,170,73}



\begin{tikzpicture}

	\tikzset{graphNode/.style = {circle, fill=ImClrNode, minimum width=\ImNodeWidth, minimum height = \ImNodeWidth, inner sep=0pt, text width=\ImNodeWidth, align=center},
    labelNode/.style = {circle, fill=white, inner sep=1pt, outer sep=3pt},
    edgeTh/.style = {stealth-, thick}}
  
  \def\energyPrices{{0,2, 1, 2, 1, 6, 16, 14, 3, 2, 5, 3, 15, 3, 2, 1, 2,0}}
	
	% Prepare coordinates
	\pgfmathsetmacro{\prepareLayers}{\ImNumInts+1};
	\foreach \y in {0,...,\prepareLayers}
	{
		\foreach \x in {0,...,\ImNumModes}
		{
			\pgfmathsetmacro{\crdX}{(\x-1) * \ImGridHor + \ImGridHor/2};
        		\pgfmathsetmacro{\crdY}{-((\y-1) * \ImGridVert + \ImGridVert/2)};        		
        		\coordinate (\x-\y) at (\crdX,\crdY); 			
		}
	}
	
	\foreach \y in {2,...,\ImNumInts} 
	{
	    \pgfmathsetmacro{\crdY}{-0.8*\y-0.4};		
	    \draw[gray, dotted] ($(1-\y) - (0.5cm,0)$) -- ($(3-\y) + (0.5cm,0)$);
	}
	
	% Draw interval labels
	\foreach \y in {2,...,\ImNumInts}
	{
        \pgfmathtruncatemacro{\lbl}{\y-1};
		\node at ($(1-\y) - (1cm,0)$) {$\Interval{\lbl}$};
	}
	
	% Draw mode labels
	\foreach \x/\lbl in {\ImOffIdx/$\StateOff$,\ImProcIdx/$\StateProc$,\ImIdleIdx/$\StateIdle$}
	{
		\node at ($(\x-1) + (0,0.5cm)$) {\lbl};
	}
	
	% Draw nodes
	\foreach \y in {2,...,\ImNumInts}
	{
		\foreach \x in {1, ...,\ImNumModes}
		{
		\node[graphNode] at (\x-\y) {};
		}
	}	
	\node[graphNode] at (\ImOffIdx-1) {};  % base off
	\node[graphNode] at (\ImOffIdx-18) {};  % base off
	
	% optimal path between I4-proc and I10-proc
	% \begin{scope}[transform canvas={yshift=0.1cm}]
	%     \draw (\ImProcIdx-9) edge[ImClrGreen, dashed, thick, shorten >=0.3cm, shorten <=0.3cm, bend left=10] (\ImOffIdx-10);
	% \end{scope}
	
	
	% \begin{scope}[transform canvas={xshift=-0.15cm}]
 %    	\draw[ImClrGreen, thick, densely dashed, shorten >=0.1cm, shorten <=0.1cm] (\ImOffIdx-10) -- (\ImOffIdx-11);
 %    	\draw[ImClrGreen, thick, densely dashed, shorten >=0.1cm, shorten <=0.1cm] (\ImOffIdx-11) -- (\ImOffIdx-12);
	% \end{scope}
	
	% \begin{scope}[transform canvas={yshift=-0.1cm}]
	%     \draw (\ImOffIdx-12) edge[ImClrGreen, thick, dashed, shorten >=0.3cm, shorten <=0.3cm, bend left=10] (\ImProcIdx-14);
	% \end{scope}
	
	% Draw edges
	% - off - off
	\foreach \i in {1,...,\ImNumInts} {
		\pgfmathsetmacro{\nxt}{1+\i};		
		\pgfmathtruncatemacro\cst{\energyPrices[\i] * 0};
		\draw[-stealth, shorten >=0.1cm, shorten <=0.1cm] (\ImOffIdx-\i) -- (\ImOffIdx-\nxt) node[labelNode, pos=0.5,anchor=west] {\scriptsize \cst};
	}
	
	% proc-proc
	\pgfmathsetmacro\maxInterval{\ImNumInts-1}
	\foreach \i in {2,...,\maxInterval} {
		\pgfmathsetmacro{\nxt}{1+\i};		
		\pgfmathtruncatemacro\cst{\energyPrices[\i] * 4};
		\draw[-stealth, shorten >=0.1cm, shorten <=0.1cm] (\ImProcIdx-\i) -- (\ImProcIdx-\nxt) node[labelNode, pos=0.5, anchor=west] {\scriptsize \cst};
	}
	
	% idle-idle
	\pgfmathsetmacro\maxInterval{\ImNumInts-1}
	\foreach \i in {2,...,\maxInterval} {
		\pgfmathsetmacro{\nxt}{1+\i};		
		\pgfmathtruncatemacro\cst{\energyPrices[\i] * 2};
		\draw[-stealth, shorten >=0.1cm, shorten <=0.1cm] (\ImIdleIdx-\i) -- (\ImIdleIdx-\nxt) node[labelNode, pos=0.5, anchor=west] {\scriptsize \cst};
	}
	
	% proc-idle
	% \foreach \i in {2,...,\ImNumInts} {		
	% 	\draw (\ImProcIdx-\i) edge[-stealth, shorten >=0.1cm, shorten <=0.1cm, out=30, in=150, looseness=0.3] node[labelNode, pos=0.5, anchor=east] {\scriptsize 0} (\ImIdleIdx-\i);
	% 	\draw (\ImIdleIdx-\i) edge[-stealth, shorten >=0.1cm, shorten <=0.1cm, out=210, in=330, looseness=0.3] node[labelNode, pos=0.5, anchor=east] {\scriptsize 0} (\ImProcIdx-\i);
	% }

    % proc-idle + idle-proc
    \pgfmathsetmacro\maxInterval{\ImNumInts-1}
	\foreach \i in {2,...,\maxInterval} {		
		\pgfmathsetmacro{\nxt}{1+\i};
		\pgfmathtruncatemacro\cst{\energyPrices[\i] * 2};
		\draw (\ImIdleIdx-\i) edge[-stealth, shorten >=0.1cm, shorten <=0.1cm, bend left=8] node[labelNode, pos=0.4] {\scriptsize \cst} (\ImProcIdx-\nxt);

        \draw (\ImProcIdx-\i) edge[-stealth, shorten >=0.1cm, shorten <=0.1cm, bend left=8] node[labelNode, pos=0.35] {\scriptsize \cst} (\ImIdleIdx-\nxt);
		
	}


    
	
	% proc - off
	\pgfmathsetmacro\maxInterval{\ImNumInts-1}
	\foreach \i in {2,...,\maxInterval} {		
		\pgfmathsetmacro{\nxt}{1+\i};
		\pgfmathtruncatemacro\cst{\energyPrices[\i] * 1};
		\draw (\ImProcIdx-\i) edge[-stealth, shorten >=0.1cm, shorten <=0.1cm, bend left=10] node[labelNode, pos=0.3] {\scriptsize \cst} (\ImOffIdx-\nxt);
		
	}
	
	% off - proc
	\pgfmathsetmacro\maxInterval{\ImNumInts-2}
	\foreach \i in {2,...,\maxInterval} {		
		\pgfmathsetmacro{\nxt}{2+\i};
		\pgfmathtruncatemacro\nxtCst{\i+1};
		\pgfmathtruncatemacro\cst{5*\energyPrices[\i] + \energyPrices[\nxtCst]*5};
		\draw (\ImOffIdx-\i) edge[-stealth, shorten >=0.1cm, shorten <=0.1cm, bend left=10] node[labelNode, pos=0.35] {\scriptsize \cst} (\ImProcIdx-\nxt);
		
	}
	
	% \node[graphNode,fill=ImClrGreen] at (2-9) {};
	% \node[graphNode,fill=ImClrGreen] at (2-14) {};
	
		
\end{tikzpicture}
}

==> fig/tikz_data/problem2_feasible_sols.tex <==
\tikzset{
  mybox A/.style={solid, fill=blue!65, draw=blue!60, fill opacity=0.45}, % LBBD base
  mybox E/.style={solid, fill=gray!65, draw=gray!60, fill opacity=0.45}, % ILP base
}

% Derived styles (same family; infeasible = lighter + hatch)
\tikzset{
  lbbd-feas/.style   ={mybox A},
  lbbd-infeas/.style ={mybox A,
                       fill=blue!25, fill opacity=0.55,
                       pattern={Lines[angle=45,distance=3pt,line width=0.35pt]},
                       pattern color=blue!60},
  ilp-feas/.style    ={mybox E},
  ilp-infeas/.style  ={mybox E,
                       fill=gray!25, fill opacity=0.55,
                       pattern={Lines[angle=45,distance=3pt,line width=0.35pt]},
                       pattern color=gray!60},
}

% Stacking reset helper (unchanged)
\makeatletter
\newcommand\resetstackedplots{%
  \pgfplots@stacked@isfirstplottrue
  \addplot [forget plot,draw=none] coordinates{(1,0) (2,0) (3,0) (4,0) (5,0) (6,0) (7,0) (8,0)};
}
\makeatother

\begin{tikzpicture}
\begin{axis}[
    width=0.9\textwidth, height=0.25\textwidth,
    ybar stacked, ymin=0,
    enlarge x limits=0.2,
    xtick={1,2,3,4,5,6,7,8},
    xticklabels={
      {Brandimarte $\alpha=0.25$},
      {Brandimarte $\alpha=0.5$},
      {Brandimarte $\alpha=0.75$},
      {Brandimarte $\alpha=1.0$},
      {Fattahi $\alpha=0.25$},
      {Fattahi $\alpha=0.5$},
      {Fattahi $\alpha=0.75$},
      {Fattahi $\alpha=1.0$}
    },
    xticklabel style={rotate=25,anchor=east,yshift=-7pt,xshift=4pt},
    ylabel={instances [-]},
    legend entries={LBBD proven feasible,LBBD no proof of feasibility,ILP proven feasible,ILP no proof of feasibility},
    legend style={at={(0.5,1.05)},anchor=south,legend columns=2,draw=none},
    grid=both, grid style={dotted},
]

% --- LBBD (left bar of each category) ---
\addplot +[bar shift=-.22cm, lbbd-feas]   coordinates {(1,8) (2,8) (3,9) (4,10) (5,19) (6,18) (7,19) (8,16)};
\addplot +[bar shift=-.22cm, lbbd-infeas] coordinates {(1,2) (2,2) (3,1) (4,0) (5,1) (6,2) (7,1) (8,4)};

% Reset the stack before switching method
\resetstackedplots

% --- ILP (right bar of each category) ---
\addplot +[bar shift=.22cm, ilp-feas]     coordinates {(1,6) (2,6) (3,6) (4,7) (5,14) (6,15) (7,15) (8,14)};
\addplot +[bar shift=.22cm, ilp-infeas]   coordinates {(1,4) (2,4) (3,4) (4,3) (5,6) (6,5) (7,5) (8,6)};

\end{axis}
\end{tikzpicture}
